Matroid Semi-Bandits in Sublinear Time

We study the matroid semi-bandits problem, where at each round the learner plays a subset of $K$ arms from a feasible set, and the goal is to maximize the expected cumulative linear rewards. Existing algorithms have per-round time complexity at least $\Omega(K)$, which becomes expensive when $K$ is large. To address this computational issue, we propose FasterCUCB whose sampling rule takes time sublinear in $K$ for common classes of matroids: $O(D\text{ polylog}(K)\text{ polylog}(T))$ for uniform matroids, partition matroids, and graphical matroids, and $O(D\sqrt{K}\text{ polylog}(T))$ for transversal matroids. Here, $D$ is the maximum number of elements in any feasible subset of arms, and $T$ is the horizon. Our technique is based on dynamic maintenance of an approximate maximum-weight basis over inner-product weights. Although the introduction of an approximate maximum-weight basis presents a challenge in regret analysis, we can still guarantee an upper bound on regret as tight as CUCB in the sense that it matches the gap-dependent lower bound by Kveton et al. (2014a) asymptotically.

==> app_unstructured.tex <==
\section{Proofs for speeding up the linear maximization \eqref{eq:combucb}}
\subsection{Proofs of Section~\ref{sec:fixed-theta}}
\begin{replemma}{lem:unstructured-Nk-v1} % version 1 by textbook
    Let $\theta>0$ and \textcolor{blue}{$\lambda_t=\sqrt{2\sigma^2\ln(t\ln^2t)}$}. 
    Define $I_{\theta}=\{k\in[K]:\mu_k<\mu_1\leq(1+\theta)\mu_k\}$ and $\gap{k}^{\theta}=\mu_1-(1+\theta)\mu_k$.
    Then, for any $k\notin I_{\theta}$ and any $\epsilon>0$, 
    \begin{equation}\tag{\ref{eq:unstructured-Nk-v1}}
    \expectation{}{N_k(T)}
    \leq \frac{2\sigma^2(1+\theta)^2}{(\gap{k}^{\theta}-\epsilon)^2}\left(\ln T + {\color{violet}c(T,\theta)})\right) + {\color{violet}\frac{2\sigma^2\ln\ln T}{\epsilon^2}},
    \end{equation}
    where $c(T,\theta)=1+\sqrt{\pi(\ln(T\ln^2 T))}+2\ln\ln T$.
\end{replemma}
\begin{proofof}{Lemma~\ref{lem:unstructured-Nk-v1}}\label{proof:unstructured-Nk-v1}
Fix any $k\notin I_{\theta}$.
By the design of Algorithm~\ref{alg:approx-uniform-matroid-cucb}, a suboptimal arm $k$ selected at time $t$ implies  
\[
\ind{\ub_k(t-1)\geq\ub_1(t-1)}
\leq
\ind{(1+\theta)v_k(t-1)\geq v_1(t-1), x_k(t)=1}.
\]
The expectation of the RHS can be bounded by the standard idea which  decouples the randomness from the behavior of Algorihtm~\ref{alg:approx-uniform-matroid-cucb} by introducing $z\in\reals$: 
\begin{align*}
N_k(T)
& \leq \sum_{t=1}^T\ind{(1+\theta)v_k(t-1)\geq\min_{s<t}\left\{\tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}\right\}, x_k(t)=1}\\
& \leq \sum_{t=1}^T\underbrace{
\ind{(1+\theta)\left(\tilde{\mu}_k(t-1)+\frac{\lambda_T}{\sqrt{t}}\right)\geq\min_{s<t}\left\{\tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}\right\}}
}_{(*)_t}
\end{align*}
where the second inequality is due to $N_k(t)-N_k(t-1)=1$ whenever $x_k(t)=1$.
By standard decoupling idea \cite{lattimore2020bandit}, we upper bound $(*)_t$ by comparing the LHS and RHS against a number $z=\mu_1-\epsilon$:
\[
{\color{blue}
(*)_t \leq \ind{(1+\theta)\left(\tilde{\mu}_k(t-1)+\frac{\lambda_T}{\sqrt{t}}\right)\geq \mu_1-\epsilon}
+\ind{\mu_1-\epsilon\geq\min_{s<t}\left\{\tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}\right\}}
}.
\]
By the $\frac{\sigma}{\sqrt{s}}$-subgaussianity of $\tilde{\mu}_k(s)$ and substituting $\lambda_t=\sqrt{2\sigma^2\ln f(t)}$, we have 
\begin{align}
    \expectation{}{\ind{\mu_1-\epsilon \geq \min_{s<t}\left\{\tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}\right\}}}
    & \leq \sum_{s<t}e^{-\frac{s\left(\epsilon+\sqrt{\frac{2\sigma^2 \ln f(t)}{s}}\right)^2}{2\sigma^2}}
    \leq \frac{2\sigma^2}{\epsilon^2f(t)},\label{eq:unstructured-Nk-part1}\\
    \quad\text{and}\quad
    \expectation{}{\ind{\frac{\gap{k}^{\theta}-\epsilon}{1+\theta}-\frac{\lambda_T}{\sqrt{t}} \leq \tilde{\mu}_k(t)-\mu_k}}
    & \leq e^{-\left(\frac{(\gap{k}^{\theta}-\epsilon)\sqrt{t/2\sigma^2}}{1+\theta}-\sqrt{\ln f(T)}\right)^2}.\label{eq:unstructured-Nk-part2}
\end{align}
In the RHS of \eqref{eq:unstructured-Nk-part2}, the exponent $\frac{(\gap{k}^{\theta}-\epsilon)\sqrt{t/2\sigma^2}}{1+\theta}-\sqrt{\ln f(T)}\geq 0$ when $t\geq t_k^{\theta}=\frac{2\sigma^2(1+\theta)^2\ln f(T)}{(\gap{k}^{\theta}-\epsilon)^2}$.
Therefore, substituting $f(t)=t\ln^2 t$ into \eqref{eq:unstructured-Nk-part1}\eqref{eq:unstructured-Nk-part2}, we evaluate
\begin{align*}
    \expectation{}{N_k(T)} 
    & \leq t_k^{\theta} +{\color{blue}\sum_{t=t_k^{\theta}+1}^T}\left(\frac{1}{f(t)}+{\color{blue}e^{-\left(\frac{(\gap{k}^{\theta}-\epsilon)\sqrt{t/2\sigma^2}}{1+\theta}-\sqrt{\ln f(T)}\right)^2}}\right)\\
    & \leq t_k^{\theta} + \frac{2\sigma^2\ln\ln T}{\epsilon^2} +{\color{blue}\frac{2\sigma^2(1+\theta)^2}{(\gap{k}^{\theta}-\epsilon)^2}\left(1+\sqrt{\pi\ln f(T)}\right)},
\end{align*}
where the second inequality is because $\sum_{t=t_k^{\theta}+1}^T\frac{2\sigma^2}{\epsilon^2t\ln^2t} \leq \frac{2\sigma^2}{\epsilon^2}\int_{\ln(t_k^{\theta}+1)}^{\ln T}\frac{dx}{x}\leq \frac{2\sigma^2}{\epsilon^2}\ln\ln T$, and an application of Lemma~\ref{lem:unstructured-int} with $\alpha=\frac{\gap{k}^{\theta}-\epsilon}{\sqrt{2\sigma^2}(1+\theta)}$ and $\beta=\sqrt{\ln f(T)}$ to bound the third term. 
The proof is completed by a simple rearrangement.
\todo[inline]{RC: not sure whether it is possible to upper bound $\sum_{t=t_k^{\theta}+1}^Te^{-\left(\frac{(\gap{k}^{\theta}-\epsilon)\sqrt{t/2\sigma^2}}{1+\theta}-\sqrt{\ln f(T)}\right)^2}$ without yielding the dependency on $\frac{2\sigma^2(1+\theta)^2}{(\gap{k}^{\theta}-\epsilon)^2}$.}
\end{proofof}

\begin{replemma}{lem:unstructured-Nk-v2} % version 2 by \cite{kveton2014matroid}
    Let $\theta>0$ and \textcolor{blue}{$\lambda_t=\sqrt{6\sigma^2\ln t}$}. 
    Define $I_{\theta}=\{k\in[K]:\mu_k<\mu_1\leq(1+\theta)\mu_k\}$ and $\gap{k}^{\theta}=\mu_1-(1+\theta)\mu_k$.
    Then, for any $k\notin I_{\theta}$, 
    \[
    \expectation{}{N_k(T)}
    \leq \frac{24\sigma^2(1+\theta)^2\ln T}{(\gap{k}^{\theta})^2} 
    + {\color{violet}\frac{1}{T} + \frac{\pi^2}{6}}.
    \]
\end{replemma}
\begin{proofof}{Lemma~\ref{lem:unstructured-Nk-v2}}\label{proof:unstructured-Nk-v2}
Fix any $k\notin I_{\theta}$.
By the design of Algorithm~\ref{alg:approx-uniform-matroid-cucb}, a suboptimal arm $k$ selected at time $t$ implies  
\[
\ind{\ub_k(t-1)\geq\ub_1(t-1)}
\leq
\ind{(1+\theta)v_k(t-1)\geq v_1(t-1), x_k(t)=1},
\]
and hence the number $N_k(T)$ of pulls of arm $k$ up to time $T$ is 
\begin{align}
N_k(T)
& \leq \sum_{t=1}^T\ind{(1+\theta)v_k(t-1)\geq\min_{s<t}\left\{\tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}\right\}, x_k(t)=1} \nonumber\\
& \leq \sum_{t=1}^T\ind{(1+\theta)\left(\tilde{\mu}_k(t-1)+\frac{\lambda_T}{\sqrt{t-1}}\right)\geq\min_{s<t}\left\{\tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}\right\}} \nonumber\\
& \leq t_k^{\theta} + \sum_{t=t_k^{\theta}}^T\sum_{s<t}\ind{(1+\theta)\left(\tilde{\mu}_k(t-1)+\frac{\lambda_T}{\sqrt{t-1}}\right)\geq \tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}},\label{eq:unstructured-Nk-truncate}
\end{align}
where the second inequality is due to $N_k(t)-N_k(t-1)=1$ whenever $x_k(t)=1$.
\textcolor{blue}{
Inspired by \cite{kveton2014matroid}, we upper bound $\ind{(1+\theta)\left(\tilde{\mu}_k(t-1)+\frac{\lambda_T}{\sqrt{t-1}}\right)\geq \tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}}$ by
\begin{equation}\label{eq:unstructured-Nk-3parts}
    \ind{\tilde{\mu}_k(t-1) \geq \mu_k + \frac{\lambda_T}{\sqrt{t-1}}}
    +\ind{\mu_1 \geq \tilde{\mu}_1(s)+\frac{\lambda_t}{\sqrt{s}}}
    +\ind{(1+\theta)\left(\mu_k+\frac{2\lambda_T}{\sqrt{t-1}}\right) > \mu_1},
\end{equation}
where the third term is 0 when $t\geq t_k^{\theta}=\frac{4(1+\theta)^2\lambda_T^2}{(\gap{k}^{\theta})^2}$.
}
By the $\frac{\sigma}{\sqrt{s}}$-subgaussianity of $\tilde{\mu}_k(s)$ and substituting $\lambda_t=\sqrt{6\sigma^2\ln t}$, we get
\begin{equation}\label{eq:unstructured-Nk-part12}
    \expectation{}{\text{the first two terms in \eqref{eq:unstructured-Nk-3parts}}}
    \leq e^{-3\ln T}+e^{-3\ln t} = \frac{1}{T^3}+\frac{1}{t^3}.
\end{equation}
Plugging \eqref{eq:unstructured-Nk-3parts}\eqref{eq:unstructured-Nk-part12} into \eqref{eq:unstructured-Nk-truncate}, we evaluate 
\begin{align*}
    \expectation{}{N_k} 
    & \leq t_k^{\theta} + \sum_{t=t_k^{\theta}}^T\sum_{s<t}\left(\frac{1}{T}+\frac{1}{t^3}\right)
    \leq t_k^{\theta} + \frac{1}{T^2} + \frac{\pi^2}{6}
\end{align*}
\end{proofof}

\begin{lemma}\label{lem:unstructured-int}
    Let $\alpha,\beta>0$. Then, $\int_0^{\infty}e^{-(\alpha\sqrt{t}-\beta)^2}dt\leq\frac{1+\beta\sqrt{\pi}}{\alpha^2}$.
    \end{lemma}
\begin{proof}
    By changing the variables $s=(\alpha\sqrt{t}-\beta)^2$ and then substituting $\frac{ds}{dt}=\frac{\alpha\sqrt{s}}{\sqrt{t}}=\frac{\alpha^2\sqrt{s}}{\sqrt{s}+\beta}$:
    \[
    \int_0^{\infty}e^{-(\alpha\sqrt{t}-\beta)^2}dt
    =\frac{1}{\alpha^2}\int_0^{\infty}\left(
        1+\frac{\beta}{\sqrt{s}}
    \right)e^{-s}ds
    \leq\frac{1+\beta\Gamma(\frac{1}{2})}{\alpha^2}
    =\frac{1+\beta\sqrt{\pi}}{\alpha^2}.
    \]
\end{proof}

\subsection{Proofs of Section~\ref{sec:varying-theta}}
\begin{proofof}{$t_k$ for choice 1}\label{proof:choice1-tk}
Here we derive the precise form for $t_k=\inf\{t\in\ints:(\gap{k}-\epsilon)\sqrt{t}\geq\sqrt{2\sigma^2\ln t}+\mu_k\}$.
For any $w\in\reals$, let $W(w)$ be the Lambert W function \cite{mezo2022lambert} which is defined as the solution to $x\exp(x)=w$.
Let $z=\sqrt{\ln t}$.
By rewriting $(\gap{k}-\epsilon)\sqrt{t}=\sqrt{2\sigma^2\ln t}+\mu_k$ as follows:
\begin{align}
    & (\gap{k}-\epsilon)\exp(z)=\sqrt{2\sigma^2}\cdot z+\mu_k\nonumber\\
    & \qquad \Leftrightarrow \left(-\left(z+\frac{\mu_k}{\sqrt{2\sigma^2}}\right)\right)\exp(-z)=-\frac{\gap{k}-\epsilon}{\sqrt{2\sigma^2}} \nonumber\\
    & \qquad \Leftrightarrow y\exp(y)=-\frac{\gap{k}-\epsilon}{\sqrt{2\sigma^2}}\cdot \exp\left(\frac{\mu_k}{\sqrt{2\sigma^2}}\right)
    \tag{let $y=-(z+\frac{\mu_k}{\sqrt{2\sigma^2}})$},
\end{align}
we get the closed-form of $t_k$: 
\begin{equation}\label{eq:basic-tk-sol}
    t_k=\left\lceil
    \exp\left(
        \left(-W\left(-\frac{\gap{k}-\epsilon}{\sqrt{2\sigma^2}}\cdot \exp\left(\frac{\mu_k}{\sqrt{2\sigma^2}}\right)\right)-\frac{\mu_k}{\sqrt{2\sigma^2}}\right)^2
        \right)
    \right\rceil.
\end{equation}
In fact, the form we solve is Lambert W function of type (0,1), see \cite{mezo2022lambert}[Sec 5.3.1].
\end{proofof}

==> sections/4.algo.tex <==
\section{Algorithm}\label{sec:algo}
\subsection{Asymptotic opt in \texorpdfstring{$D\polylog{T}$ time}{Dpolylog(T)-time}}\label{sec:fixed-theta}
\paragraph{Naoto's algorithm.}
Initially, construct $\bin{q,r}(\theta)=(a(1+\theta)^{q-1},a(1+\theta)^q]\times((1+\theta)^{r-1},(1+\theta)^r]$ for $(q,r)\in\{1,\cdots,\lceil\log_{1+\theta}\frac{b}{a}\rceil\}\times\{1,\cdots,\lceil\log_{1+\theta}\sqrt{\abs{\decls_0}}\rceil\}$, where $\decls_0=\{\istar{\be_k}:k\in[K]\}$.
At each time, take top-$D$ by sorting the bins, and then expand the bins.
\begin{itemize}
    \item Initial bins construction: $\bigO(K\ln K+K(\log_{1+\theta}\frac{b}{a}+\log_{1+\theta}\sqrt{\abs{\decls_0}}))$
    \item At each time $t$, $(1+\theta)$-approx solution to \eqref{eq:combucb} can be computed by sorting the bins, taking top-$D$ arms, and updating the chosen $D$ arms.
    If $a$ and $b$ are universal constants, then the per-round time complexity is 
    \begin{align*}
        & \bigO\left(\log_{1+\theta}^2\frac{b}{a}\log_{1+\theta}^2\sqrt{t}+D(\log_{1+\theta}\frac{b}{a}+\log_{1+\theta}\sqrt{t})\right)\\
        & \quad =\bigO\left(\log_{1+\theta}^2t+D\log_{1+\theta}t\right)
        \leq \bigO((\theta^{-2}+D\theta^{-1})\ln t),
    \end{align*}
    where the last inequality is because $\frac{x}{1+x}\leq\ln(1+x)$ holds for any $x>-1$.
\end{itemize}
By substituting $\theta=\frac{1}{\ln^m T}$, the amortized time is
\[
\frac{\sum_{t=1}^T(\ln^{2m+1} t+D\ln^{m+1}t)}{T}\leq \frac{\int_0^{\ln T}(x^{2m+1}+Dx^{m+1})e^xdx}{T}=\bigO(\ln^{2m+1}T+D\ln^{m+1}T).
\]

\paragraph{Notation.}
Let $v_k(t-1)=\hat{\mu}_k(t-1)+\frac{\lambda_t}{\sqrt{N_k(t-1)}}$ denote the UCB index of arm $k$ at round $t$, and $\ub_k(t-1)$ be a $(1+\theta)$-approx to $v_k(t-1)$ such that 
\[
\frac{\ub_k(t-1)}{1+\theta}\leq v_k(t-1)\leq\ub_k(t-1).
\]
In addition to $\hat{\mu}_k(t)$, we define $\tilde{\mu}_k(t)$ as the average of $t$ independent r.v.'s from $\nu_k$.
